Challenges and Opportunities of Teaching Data Visualization Together with Data Science

With the increasing amount of data globally, analyzing and visualizing data are becoming essential skills across various professions. It is important to equip university students with these essential data skills. To learn, design, and develop data visualization, students need knowledge of programming and data science topics. Many university programs lack dedicated data science courses for undergraduate students, making it important to introduce these concepts through integrated courses. However, combining data science and data visualization into one course can be challenging due to the time constraints and the heavy load of learning. In this paper, we discuss the development of teaching data science and data visualization together in one course and share the results of the post-course evaluation survey. From the survey's results, we identified four challenges, including difficulty in learning multiple tools and diverse data science topics, varying proficiency levels with tools and libraries, and selecting and cleaning datasets. We also distilled five opportunities for developing a successful data science and visualization course. These opportunities include clarifying the course structure, emphasizing visualization literacy early in the course, updating the course content according to student needs, using large real-world datasets, learning from industry professionals, and promoting collaboration among students.

==> Files/RelatedWork.tex <==
\section{Related Work}

In today's information age, both data science and data visualization are essential for effectively communicating information~\cite{Eltweri2022Big}. These fields are rapidly growing in both academia and industry~\cite{Sean2019DS}. As these fields continue to expand, equipping students with the necessary data science and data visualization skills is crucial~\cite{Mike2023Birth}. 
%Data literacy encompasses the ability to categorize, collect, clean, preprocess, and analyze data, as well as the ability to read, critically review, interact effectively, and carefully design and develop data visualizations~\cite{Inverarity2022literacy}. 
The importance of data science education can be seen in the increasing number of dedicated journals, such as the Journal of Statistics and Data Science Education\cite{JSDSE2024}, conferences, such as the International Conference on Big Data Analytics~\cite{ieee2023icbda} and workshops, such as the National Workshop on Data Science Education~\cite{cdss2023workshop} and IEEE Data Science and Learning Workshop.~\cite{dslw2022}. Similarly, the growing importance of visualization education is evident in the proliferation of dedicated workshops such as Eduvis~\cite{eduvis2023}, VisGuides~\cite{AbdulRahman2020, Bach2022}, VisFutures~\cite{Perin2020}, and VisActivities~\cite{Huron2020, Huron2021}, as well as the rise in textbooks~\cite{munzner2014visualization, kirk2019data, cairo2012functional}. Recent research has also stressed the urgency of research and discussion on data visualization education through a call to action~\cite{Bach2024call}.

Several research efforts have been conducted in the area of data science education. For instance, some researchers have conducted systematic reviews and analyzed different data science courses offered at various universities~\cite{Wu2017review, Sean2019DS}. Some research has focused on designing new data science curricula~\cite{Bina2016course, BRUNNER2016course} or integrating data science with introductory-level computing courses~\cite{Bart2018DScourse}. Other studies have tailored data science courses to specific domains such as bioinformatics~\cite{Via2013Bio} and statistics~\cite{Hardin2015stat}. Similarly, various studies have explored different approaches to teaching data visualization, including teaching in multiple methods~\cite{Niemann2023multiple}, project-based learning~\cite{Dietrich2021project}, and activity or tutorial-based learning~\cite{Lo2019tutorial, Knudsen2023activity}, reflecting the evolving strategies educators use to improve visualization literacy among students.

However, these efforts often remain isolated within their respective disciplines, lacking integration across data science and visualization. To address this gap, there is a need for introductory courses that combine both disciplines, ensuring students gain a holistic understanding and skill set.   Also, current research in data science and data visualization education predominantly reflects the educator's viewpoint, often drawn from insights provided by instructors and teaching assistants, many of whom are PhD candidates. However, these educators, no longer in the student role, may not fully grasp the students' current experiences and needs. Understanding the student's perspective is crucial for effectively redesigning courses to better align with their evolving needs and requirements. Therefore, there is a need to gather and analyze student perspectives following course completion.

==> Files/RelatedWork_old.tex <==
\section{Related work}
\subsection{Data science education}
The field of data science is growing in importance, both in academia and industry~\cite{Sean2019DS}. As it continues to expand, it is essential to prepare students with the necessary data science skills~\cite{Mike2023Birth}. This has led to a greater focus on data science education. The importance of data science education is further evidenced by the growing number of dedicated journals, such as the Journal of Statistics and Data Science Education~\cite{JSDSE2024}, as well as conferences such as the International Conference on Big Data Analytics\cite{ieee2023icbda} and workshops such as the National Workshop on Data Science Education~\cite{cdss2023workshop} and IEEE Data Science and Learning Workshop.~\cite{dslw2022}

Various research efforts have been conducted related to data science education. For example, a few researchers conducted systematic reviews and analyzed different data science courses offered at universities~\cite{Wu2017review, Sean2019DS}. Some research has focused on designing new data science curricula~\cite{Bina2016course, BRUNNER2016course} or integrating data science with introductory-level computing courses~\cite{Bart2018DScourse}. Other studies have tailored data science courses to specific domains such as bioinformatics~\cite{Via2013Bio} and statistics~\cite{Hardin2015stat}. Most of these studies concentrate on course development, instructor reflections, or experience reports, providing guidelines for future courses based on lessons learned during their implementation.

Despite these contributions, a notable gap remains in addressing student perspectives on data science courses. Understanding the student's viewpoint is crucial for redesigning courses to better align with their needs and requirements. This gap highlights the need for studies that gather and analyze student feedback on data science courses.

\subsection{Data visualization education}

In today's information age, visualizations play a critical role in effectively communicating information. Visualization literacy, which encompasses the ability to read, interpret, create, and critically evaluate data visualizations, has become an essential skill. This increasing importance is evident in the proliferation of workshops focused on visualization education, such as Eduvis'23. Additionally, the rise in textbooks, software tools, and courses dedicated to visualization education underscores the field's growing significance. Recent calls to action highlight the urgency of research and discussion on data visualization education.

Various studies have explored different approaches to teaching data visualization, including multi-method courses, project-based learning, and tutorial-based instruction. These efforts reflect the evolving strategies educators use to improve visualization literacy among students. However, most of these studies focus solely on data visualization. Data visualization is a complex discipline that requires knowledge of various fields, including data science.  To teach data visualization effectively, it is crucial to introduce data science as well.  Many universities have not previously offered data science courses to undergraduate students, making it essential to design an introductory course that combines both data science and data visualization. 

A notable gap in the existing research is the predominant focus on the educator's perspective, often derived from insights provided by instructors and teaching assistants (many of whom are PhD students). These educators, who are no longer in the student role, may not fully capture the current student experience and needs. Therefore, understanding the student's perspective is equally important. Gathering and analyzing student feedback after course completion is essential for redesigning courses to meet students' needs and requirements better.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.

